Remote Estimation of the Wiener Process over a Channel with Random Delay

In this paper, we consider a problem of sampling a Wiener process, with samples forwarded to a remote estimator via a channel that consists of a queue with random delay. The estimator reconstructs a real-time estimate of the signal from causally received samples. Motivated by recent research on age-of-information, we study the optimal sampling strategy that minimizes the mean square estimation error subject to a sampling frequency constraint. We prove that the optimal sampling strategy is a threshold policy, and find the optimal threshold. This threshold is determined by the sampling frequency constraint and how much the Wiener process varies during the channel delay. An interesting consequence is that even in the absence of the sampling frequency constraint, the optimal strategy is not zero-wait sampling in which a new sample is taken once the previous sample is delivered; rather, it is optimal to wait for a non-zero amount of time after the previous sample is delivered, and then take the next sample. Further, if the sampling times are independent of the observed Wiener process, the optimal sampling problem reduces to an age-of-information optimization problem that has been recently solved. Our comparisons show that the estimation error of the optimal sampling policy is much smaller than those of age-optimal sampling, zero-wait sampling, and classic uniform sampling.

==> sec_related_work.tex <==
% !TEX root = ./sampling_BM.tex
\subsection{Related Work}



On the one hand, the results in this paper are closely related to those in \cite{2015ISITYates,SunInfocom2016,report_AgeOfInfo2016}. Both of these references considered update policies for minimizing the Age-of-information, where update times depend only on the history of the delay process. The discovery of the sub-optimality of a zero-wait policy can be found in these references.

There is a rich literature on remote estimation, e.g., \cite{mehra76, imer2010, nayyar2013, wu2013}. Optimal transmission scheduling of sensor measurements for estimation of a stochastic process was recently studied in \cite{GaoCDC2015, GaoACC2016},  which adopted a finite-horizon formulation with a bound on the total number of transmissions that the sensor can make, over a channel with transmission cost or additive noise. A result in these papers that resonates with ours is the discovery that, under a noisy channel (in contrast to a noiseless one) it may be the case that the sensor does not use all available transmission opportunities. 

In the absence of channel delay and queueing (i.e., $Y_i=0$), the problem   has been addressed
 in \cite{Astrom2002,Basar2014} and the optimality of a threshold policy established. 
As there is no channel delay in the model in \cite{Basar2014},  the problem analyzed therein is a special case of ours with $Y_i$ set to zero for all $i$.  
 
% extend their results to general $Y_i$ and also analyze signal-independent sampling.

%On the other hand, the paper is an extension of the work in \cite{Basar2014}, which considered optimal sampling of a Wiener Process for reconstruction. To our knowledge, this is the first reference that shows that the optimal sampling policy is a threshold policy.  As there is no channel delay in the model in \cite{Basar2014},  the problem analyzed therein is a special case of ours with $Y_i$ set to zero for all $i$. 



==> sec_solution_short.tex <==
% !TEX root = ./sampling_BM.tex


%In this section, we develop a simple optimal sampling policy for solving \eqref{eq_DPExpected}. % by using  martingale, Lagrangian duality, and  optimal stopping theories. % \cite{Shiryaev1978}.

%propose a simple sampling policy and show that it is optimal for 

%Somewhat surprisingly, we find that it is possible to obtain a solution that is optimal for solving \eqref{eq_DPExpected}. % has some nice structural properties that can be exploited to obtain the optimal sample policy. 

% in the sequel.
%In this section, we will solve \eqref{eq_DPExpected} by using 
%\subsection{Problem Simplification} % 
%\begin{lemma}
%Let $S\leq T$ be two stopping times of the Wiener process $W_t$ and $\mathbb{E}[T]<\infty$. Then
%\begin{align}
%\mathbb{E}\left[ W_t^4 \right] = \mathbb{E}\left[ W_s^4 \right] + \mathbb{E}\left[ (W_t- W_s)^4 \right].  
%\end{align}
%\end{lemma}
%If a sample is stored in the queue, it becomes stale while waiting for its transmission opportunity. 
%A better method is to wait until the channel becomes idle, and then generate a new sample. This completely eliminates the waiting time wasted in the queue, and hence the queue is kept empty. 
%
%\begin{lemma}\label{lem_zeroqueue}
%In \eqref{eq_DPExpected}, it is better to take samples only when the channel is idle. 
%\end{lemma}
%\begin{proof}
%See Appendix \ref{app_zeroqueue}. 
%\end{proof}
%By Lemma \ref{lem_zeroqueue}, we only need to consider a sub-class of sampling policies $\Pi_1\subset\Pi$ such that each  sample is generated and submitted to the channel after all previous samples are delivered, i.e., 
%\begin{align}
%\Pi_1 = \{\pi\in\Pi: S_{i} = G_{i} \geq D_{i-1} \text{ for all $i$}\}. \nonumber
%\end{align}%In particular, sample $i$ is delivered before sample $i+1$ is generated and sent out, i.e., $D_{i} \leq S_{i+1} = G_{i+1}$. 
%Hence, the \emph{information} that is available for determining $S_i$ includes the history of signal values $(W_t: t\in[0, S_i])$ and the transmission delays  $(Y,\ldots, Y_{i-1})$ of previous samples. To characterize this statement precisely, let us define the $\sigma$-field $\mathcal{F}_t = \sigma(W_s: s\in[0, t])$. Then, $\{\mathcal{F}_t,t\geq0\}$ is the {filtration} (i.e., a growing family of $\sigma$-fields) of the Wiener process $W_t$.
%%, and $\{\mathcal{F}_C (i), i = 1,2,\ldots\}$ is the \emph{filtration} of the channel transmission process. Then, 
%Given the transmission  durations $(Y,\ldots, Y_{i-1})$ of previous samples, $S_{i} $ is a \emph{stopping time} with respect to the filtration $\{\mathcal{F}_t,t\geq0\}$ of the Wiener process $W_t$, that is
%\begin{align}
%[\{S_{i}\leq t\} | Y,\ldots, Y_{i-1}] \in \mathcal{F}_t.\label{eq_stopping}
%\end{align}  
%Then, the policy space $\Pi_1$ can be expressed as
%\begin{align}\label{eq_policyspace}
%\!\!\!\!\Pi_1 = & \{S_i : [\{S_{i}\leq t\} | Y,\ldots, Y_{i-1}] \in \mathcal{F}_t, \nonumber\\
%&\text{$T_i$ is a regenerative process} \}.\!\!
%\end{align}  
%%This %interpretation 
%% which will be used to simplify \eqref{eq_DPExpected}:
%% for simplifying \eqref{eq_DPExpected}. %  which we obtain  the following result:
%%This interpretation motivated us to 
%
%Using the stopping times and martingale theory of Wiener process, we obtain the following  lemma 
%%
%that is useful for simplifying \eqref{eq_DPExpected}: %that is obtained along this direction 
%%is the following lemma:
%\begin{lemma}\label{lem_stop}
%Let $\tau \geq0$ be a stopping time of the Wiener process $W_t$ with $\mathbb{E}[\tau^2]<\infty$, 
%then
%\begin{align}\label{eq_stop}
%%\mathbb{E}\left[\int_0^T [{x}(0)-W_t]^2dt\right] = \mathbb{E}[T] \sigma^2.
%\mathbb{E}\left[\int_0^\tau W_t^2 dt\right]= \frac{1}{6}\mathbb{E}\left[ W_\tau^4 \right].
%\end{align}
%\end{lemma}
%\begin{proof}
%See Appendix \ref{applem_stop}.
%\end{proof}
%
%%From \eqref{eq_esti}, we can get
%%\begin{align}%\label{eq_integral}
%%\mathbb{E}\!\left\{
%%\!\int_{D_{i}}^{D_{i+1}} \!\![W_t\!-\!\hat W_t]^2dt\right\}\!{=} \mathbb{E}\!\left\{\!\int_{D_{i}}^{D_{i+1}} \! \![W_t\!-\!B(S_{i})]^2dt\right\}\!.\! \nonumber
%%\end{align}
%
%
%Let $Z_i = S_{i+1} - D_{i}\geq0$ represent the \emph{waiting time} between the delivery time $D_{i}$ of sample $i$  and the generation time $S_{i+1}$ of sample $i+1$. Then,
%$S_i =  Z_{0} +\sum_{j=0}^{i-1} (Y_{j} + Z_j)$ and $D_i =  \sum_{j=0}^{i-1} (Z_{j}+Y_{j+1})$. If $(Y,Y_2,\ldots)$ is given, $(S_0,S_1,\ldots)$ is uniquely determined by $(Z_0,Z_1,\ldots)$. Hence, one can also use $\pi = (Z_0,Z_1,\ldots)$ to represent a sampling policy. 
%% For the convenience of later discussions, we will use $\pi = (Z_0,Z_1,\ldots)$ to represent a sampling policy in the sequel. 
%%Let 
%%\begin{align}\label{eq_shift}
%%W_{s+t}-W_{s} = W_{s+t}-W_s, ~s,t\geq0,
%%\end{align}
%%represent the signal variation since time $s$. According to  \cite[Theorem 2.16]{BMbook10}, $W_{s+t}-W_{s}$ is also a  Wiener process, called \emph{time-shifted Wiener process}. 
%
%
%%  we can show that for every $i = 1,2,\ldots$,
%%\begin{align}\label{eq_integral}
%%&\mathbb{E}\left\{\int_{D_{i}}^{D_{i+1}} [W_t-\hat W_t]^2dt\right\} \nonumber\\
%%%=& \mathbb{E}\left\{\int_{D_{i}}^{D_{i+1}} [W_t-B(S_i)]^2dt\right\} \nonumber\\
%%%= & \mathbb{E}\left\{\int_{Y_i}^{Y_i+Z_i+Y_{i+1}} W_t^2dt\right\} \nonumber\\
%%%= & \frac{1}{6}\mathbb{E}\left[ B(Y_i+Z_i+Y_{i+1})^4 \right] - \frac{1}{6}\mathbb{E}\left[ B(Y_i)^4 \right] \nonumber\\
%%= & \frac{1}{6}\mathbb{E}\left[ (W_{S_{i}+Y_i+Z_i}-W_{S_i})^4 \right] + \mathbb{E}\left[Y_i + Z_i \right] \mathbb{E}\left[Y_i \right],  
%%\end{align}
%%which is proven in Appendix \ref{app_integral}.
%%%%In addition, the following result is crucial for simplifying : 
%%%\begin{lemma}\label{lem_ergodic}
%%%For the Wiener process $W_t$, if $\{S_{i+1}-S_i, i = 0,1,\ldots\}$ is ergodic, then $\{B(S_{i+1})-B(S_i), i = 0,1,\ldots\}$ is ergodic.
%%%\end{lemma}
%%%\begin{proof}
%%%%For notational simplicity, denote $C_i = S_{i+1}-S_i$ and $D_i = B(S_{i+1})-B(S_i)$. 
%%%Because of Kolmogorov's extension theorem \cite[Theorem A.3.1]{Durrettbook10}, there exists a probability space $(\Omega, \mathcal{F}, P)$ with $\Omega = \mathbb{R}^{\{0,1,\ldots\}}$ and $\omega= (\omega_0, \omega_1,\ldots)\in \Omega$ such that the sequence $C_i(\omega) = \omega_i$ has the same distribution as that of $\{S_{i+1}-S_i, i=0,1,\ldots\}$. 
%%%Let $\varphi: \Omega \mapsto \Omega$ be the shift operator such that $\varphi(\omega_0, \omega_1,\ldots) = (\omega_1, \omega_2,\ldots)$, and let $C(\omega) = \omega_0$. Hence, $C_i(\omega) = C(\varphi^i \omega)$. Because $\{S_{i+1}-S_i, i = 0,1,\ldots\}$ is ergodic, $\varphi$ is measure preserving, i.e., $P[\varphi^{-1} A] = P[A]$ for all $A\in \mathcal{F}$.
%%%%Then,   measurable mapping $$ such that   where $C$ is a random variable. 
%%%
%%%See Appendix \ref{applem_ergodic}.
%%%\end{proof}
%%%Because the $Y_i$'s are \emph{i.i.d.} and 
%%Because $T_i $ is a regenerative process, the renewal theory \cite{Ross1996} tells us that $\frac{1}{n} 
%%\mathbb{E}[S_n]= \frac{1}{n} 
%%\sum_{i=1}^n \mathbb{E}\left[Y_i+Z_i\right]$ is a convergent seqence and %$(Z_1,Z_2,\ldots)$ is also stationary and ergodic. Hence, 
%%%Because  $(Y,Y_2,\ldots)$ are \emph{i.i.d.} and $(Z_1,Z_2,\ldots)$ are stationary and ergodic, we can obtain
%%\begin{align}
%%&\limsup_{T\rightarrow \infty}\frac{1}{T}\mathbb{E}\left\{\int_0^{T} [W_t-\hat W_t]^2dt\right\} \nonumber
%%\\
%%=& \lim_{n\rightarrow \infty}\frac{\mathbb{E}\left\{\int_0^{D_n} [W_t-\hat W_t]^2dt\right\}}{\mathbb{E}[D_n]} \nonumber\\
%%=& \lim_{n\rightarrow \infty}\frac{\sum_{i=1}^n\!\! \left\{\mathbb{E}\left[(W_{S_{i}+Y_i+Z_i}\!-\!W_{S_i})^4\right]\!+\! 6\mathbb{E}\left[Y_i+Z_i\right]\mathbb{E}\left[Y_i\right]\right\}}{6\sum_{i=1}^n \mathbb{E}\left[Y_i+Z_i\right]}\nonumber\\
%%= & \lim_{n\rightarrow \infty}\frac{\sum_{i=1}^n\mathbb{E}\left[(W_{S_{i}+Y_i+Z_i}-W_{S_i})^4\right]}{ 6\sum_{i=1}^n \mathbb{E}\left[Y_i+Z_i\right]} +  \mathbb{E}\left[Y\right],\nonumber
%%\end{align}
%%where we have used $\mathbb{E}\left[D_n\right]=\mathbb{E}[\sum_{i=0}^{n-1} (Z_{i}+Y_{i+1})] = \mathbb{E}[\sum_{i=0}^{n-1} (Y_{i}+Z_{i})]$ and $\mathbb{E}\left[Y_i\right] = \mathbb{E}\left[Y\right]$.
%%Hence, 
%Using Lemma \ref{lem_stop}, \eqref{eq_DPExpected} can be rewritten as the following Markov decision process:
%\begin{align}\label{eq_Simple}
%&\min_{\pi\in\Pi_1} \lim_{n\rightarrow \infty}\frac{\sum_{i=1}^n\mathbb{E}\left[(W_{S_{i}+Y_i+Z_i}-W_{S_i})^4\right]}{ 6\sum_{i=1}^n \mathbb{E}\left[Y_i\!+\!Z_i\right]} \!+\!  \mathbb{E}\left[Y\right] \\
%&~\text{s.t.}~\lim_{n\rightarrow \infty} \frac{1}{n} 
%\sum_{i=1}^n \mathbb{E}\left[Y_i+Z_i\right]\geq \frac{1}{f_{\max}},\nonumber
%\end{align}
%where ${\mathsf{mmse}}_{\text{opt}}$ is the optimal  value of \eqref{eq_Simple}. 
%
%
%\subsection{Dual Decomposition with Zero Duality Gap}
%In order to solve \eqref{eq_Simple}, let us consider the following Markov decision process with a parameter $c\geq 0$:
%%In order to solve \eqref{eq_Simple}, let us consider the following Markov decision with a parameter $c$:
%\begin{align}\label{eq_SD}
%\!\!\!\!\!\!f(c)\!=\!\min_{\pi\in\Pi_1}&\lim_{n\rightarrow \infty}\frac{1}{n}\sum_{i=1}^n\!\mathbb{E}\!\left[\frac{1}{6}(W_{S_{i}+Y_i+Z_i}\!-\!W_{S_i})^4\!-\! c(Y_i\!+\!Z_i)\!\right]\!\!\!\!\\
%\text{s.t.}~&\lim_{n\rightarrow \infty} \frac{1}{n} 
%\sum_{i=1}^n \mathbb{E}\left[Y_i+Z_i\right]\geq \frac{1}{f_{\max}},\nonumber
%\end{align}
%where $f(c)$ is the optimum  value of \eqref{eq_SD}. 
%\begin{lemma} \label{lem_ratio_to_minus}
%The following assertions are true:
%\begin{itemize}
%\vspace{0.5em}
%\item[(a).] \emph{${\mathsf{mmse}}_{\text{opt}} \gtreqqless c +  \mathbb{E}\left[Y\right]$} if and only if $f(c)\gtreqqless 0$. 
%\vspace{0.5em}
%\item[(b).] If $f(c)=0$, the solutions to \eqref{eq_Simple}
%and \eqref{eq_SD} are identical. 
%\end{itemize}
%\end{lemma}
%\begin{proof}
%See Appendix \ref{app_ratio_to_minus}.
%\end{proof}
%Hence, the solution to \eqref{eq_Simple} can be obtained by solving \eqref{eq_SD} and seeking a parameter $c\geq 0$ such that 
%\begin{align}\label{eq_c}
%f(c)=0.
%\end{align}
%
%Although \eqref{eq_SD} is not a convex optimization problem, it is possible to use the Lagrangian dual approach to solve \eqref{eq_SD} and show that it admits no duality gap. 
%
%%Specifically, define the following Lagrangian function
%%\begin{align}
%%& L(\pi;\lambda) \nonumber\\
%%=& \lim_{n\rightarrow \infty}\frac{1}{n}\sum_{i=1}^n\mathbb{E}\left[\frac{1}{6}(W_{S_{i}+Y_i+Z_i}-W_{S_i})^4\!-\! (c+\lambda)(Y_i\!+\!Z_i)\right] \nonumber\\
%%&+ \frac{\lambda}{f_{\max}}.\nonumber
%%\end{align}
%%Let
%%\begin{align}\label{eq_primal}
%%g(\lambda) = \inf_{\pi\in\Pi_1}  L(\pi;\lambda).
%%\end{align}
%%Then, the Lagrangian dual problem of \eqref{eq_SD} is defined by
%%\begin{align}\label{eq_dual}
%%\max_{\lambda\geq 0}g(\lambda).
%%\end{align}
%%Similar with \cite{Yu2006,Luo2008}, strong duality can be established as
%%\begin{lemma}\label{thm_zero_gap}
%%The optimal values of \eqref{eq_SD} and \eqref{eq_dual} are equal; i.e., their duality gap is zero.
%%\end{lemma}
%%\begin{proof}
%%See Appendix \ref{app_zero_gap}.
%%\end{proof}
%Define the $\sigma$-field $\mathcal{F}^{s}_t = \sigma(W_{s+v}-W_{s}: v\in[0, t])$ and the {filtration} $\{\mathcal{F}^{s}_t,t\geq0\}$ of the {time-shifted Wiener process} $\{W_{s+t}-W_{s},t\in[0,\infty)\}$. In addition, define ${\mathfrak{M}}_s$ as the set of square-integrable stopping times of $\{W_{s+t}-W_{s},t\in[0,\infty)\}$, i.e.,
%\begin{align}
%\mathfrak{M}_{s} = \{\tau \geq 0:  \{\tau\leq t\} \in \mathcal{F}^{s}_t, \mathbb{E}\left[\tau^2\right]<\infty\}.\nonumber
%\end{align}
%Let 
%\begin{align}
%\beta = 3(c + \lambda).\nonumber
%\end{align}
%By using Lemma \ref{lem_ratio_to_minus}, Lemma \ref{thm_zero_gap}, and the sufficient statistics of the Markov decision process \eqref{eq_primal}, we get
%\vspace{-1em}
\section{Proof Sketch of the Main Result}\label{sec_proof}
A proof sketch of Theorem~\ref{thm_1} is provided here, and the detailed proof is relegated to our technical report \cite{Sun_reportISIT17}: 

We first provide a lemma that is crucial for simplifying \eqref{eq_DPExpected}.

\begin{lemma}\label{lem_zeroqueue}
%In the optimal sampling problem \eqref{eq_DPExpected} for minimizing the MMSE of the Wiener process, it is suboptimal to take a new sample before the previous sample is delivered. 
In the optimal sampling problem \eqref{eq_DPExpected} for minimizing
the MMSE of the Wiener process, it is suboptimal to take a new sample before the previous sample is delivered.
%In the optimal sampling problem \eqref{eq_DPExpected} for minimizing the MMSE of the Wiener process, it is better to wait until the channel becomes idle, and then generate each new sample and immediately send it out.
\end{lemma}

%Unless it arrives at an empty system, sample $i$ needs to wait  in the queue until its transmission starts. 

{\blue In recent studies on age-of-information  \cite{SunInfocom2016,report_AgeOfInfo2016}, Lemma \ref{lem_zeroqueue} was intuitive and hence was used without a proof: If a sample is taken when the channel is busy, it needs to wait in the queue until its transmission starts, and becomes stale while waiting. A better method is 
to wait until the channel becomes idle, and then generate a new
sample, as stated in Lemma \ref{lem_zeroqueue}. However, this lemma is not intuitive in the MMSE minimization problem \eqref{eq_DPExpected}: The proof of Lemma \ref{lem_zeroqueue} relies on the strong Markov property of Wiener process, which may not hold for other signal processes. 
}
%\begin{proof}
%See Appendix \ref{app_zeroqueue}. 
%\end{proof}

By Lemma \ref{lem_zeroqueue}, we only need to consider a sub-class of sampling policies $\Pi_1\subset\Pi$ defined by 
%such that each  sample is generated and submitted to the channel after all previous samples are delivered, i.e., 
\begin{align}
\Pi_1 = \{\pi\in\Pi: S_{i+1} = G_{i+1} \geq D_{i} \text{ for all $i$}\}. \nonumber
\end{align}
This completely eliminates the waiting time wasted in the queue, and hence the queue should always be kept empty.
Let $Z_i = S_{i+1} - D_{i}\geq0$ represent the \emph{waiting time} between the delivery time $D_{i}$ of sample $i$  and the generation time $S_{i+1}$ of sample $i+1$. Then,
$S_i =  Z_{0} +\sum_{j=1}^{i-1} (Y_{j} + Z_j)$ and $D_i =  \sum_{j=0}^{i-1} (Z_{j}+Y_{j+1})$ for each $i=1,2,\ldots$ If $(Y_1,Y_2,\ldots)$ is given, $(S_0,S_1,\ldots)$ is uniquely determined by $(Z_0,Z_1,\ldots)$. Hence, one can also use $\pi = (Z_0,Z_1,\ldots)$ to represent a sampling policy. 

Because $T_i $ is a regenerative process, \eqref{eq_DPExpected} can be reformulated as the following Markov decision problem:
\begin{align}\label{eq_Simple}
{\mathsf{mmse}}_{\text{opt}}\triangleq&\min_{\pi\in\Pi_1} \lim_{n\rightarrow \infty}\frac{\sum_{i=0}^{n-1}\mathbb{E}\left[\int_{D_{i}}^{D_{i+1}} (W_t\!-\!W_{S_{i}})^2dt\right]}{\sum_{i=0}^{n-1} \mathbb{E}\left[Y_i+Z_i\right]} \\
&~\text{s.t.}~\lim_{n\rightarrow \infty} \frac{1}{n} 
\sum_{i=0}^{n-1} \mathbb{E}\left[Y_i+Z_i\right]\geq \frac{1}{f_{\max}},\label{eq_Simple_constraint}
\end{align}



Define the $\sigma$-fields $\mathcal{F}^{s}_t = \sigma(W_{s+v}-W_{s}: v\in[0, t])$ and $\mathcal{F}^{s+}_t = \cap_{v>t} \mathcal{F}^{s}_v$, as well as the {filtration} (i.e., a non-decreasing and right-continuous  family of  $\sigma$-fields) $\{\mathcal{F}^{s+}_t,t\geq0\}$ of the {time-shifted Wiener process} $\{W_{s+t}-W_{s},t\in[0,\infty)\}$. Let ${\mathfrak{M}}_s$ denote the set of square-integrable stopping times of $\{W_{s+t}-W_{s},t\in[0,\infty)\}$, i.e.,
\begin{align}
\mathfrak{M}_{s} = \{\tau \geq 0:  \{\tau\leq t\} \in \mathcal{F}^{s+}_t, \mathbb{E}\left[\tau^2\right]<\infty\}.\nonumber
\end{align}
After some manipulations, we formulate the Lagrangian dual problem of \eqref{eq_Simple}, which can be 
decomposed into a sequence of \emph{mutually independent} per-sample control problem \eqref{eq_opt_stopping}:
\begin{align}\label{eq_opt_stopping}
Z_i =&  \min_{\tau  \in \mathfrak{M}_{S_i+Y_i}} \mathbb{E}\left[\frac{1}{2}(W_{S_{i}+Y_i+\tau}-W_{S_i})^4\right.\nonumber\\
&~~~~~~~~~~~~~~~~\left.- {\beta}(Y_i+\tau)\bigg|W_{S_{i}+Y_i}-W_{S_i},Y_i \right],
\end{align}
where $\beta\geq0$ is the dual variable. In the proof of \eqref{eq_opt_stopping}, we have used 
%Next, by using the stopping times and martingale theory of Wiener process, we obtain 
the following lemma: 
%
%that is useful for rewritten \eqref{eq_DPExpected} as a Markov decision process without integral: %that is obtained along this direction 
%is the following lemma:
\begin{lemma}\label{lem_stop}
Let $\tau \geq0$ be a stopping time of the Wiener process $W_t$ with $\mathbb{E}[\tau^2]<\infty$, 
then
\begin{align}\label{eq_stop}
%\mathbb{E}\left[\int_0^T [{x}(0)-W_t]^2dt\right] = \mathbb{E}[T] \sigma^2.
\mathbb{E}\left[\int_0^\tau W_t^2 dt\right]= \frac{1}{6}\mathbb{E}\left[ W_\tau^4 \right].
\end{align}
\end{lemma}

Using the optimal stopping rule developed in \cite{Shiryaev1978}, we get 
\begin{theorem}
An optimal solution to \eqref{eq_opt_stopping} is
\begin{align}\label{eq_opt_stop_solution1}
Z_i = \inf \left\{ t \geq 0:\! \left|W_{S_i+Y_i+t}-W_{S_i}\right| \geq \sqrt{\beta}\right\}.
\end{align}
\end{theorem}
Notice that \eqref{eq_opt_stop_solution1} is equivalent to \eqref{eq_opt_solution}. 
\begin{theorem}\label{thm_zero_gap}
The following assertions are true:
\begin{itemize}
\item[(a).] The duality gap between \eqref{eq_Simple} and its Lagrangian dual problem is zero.
\item[(b).] A common optimal solution to \eqref{eq_DPExpected} and  \eqref{eq_Simple} is given by \eqref{eq_opt_solution} and \eqref{eq_thm1}. 
\end{itemize}
%Hence, the MMSE-optimal  policy in \eqref{eq_opt_solution} and \eqref{eq_thm1} is an optimal solution to \eqref{eq_SD}. 
\end{theorem}
By this, Theorem~\ref{thm_1} is proven.
%the duality gap between \eqref{eq_Simple} and its Lagrangian dual problem is zero, and the optimal $\beta$ is determined by \eqref{eq_thm1}. 


\ignore{



\begin{theorem}\label{thm_solution_form}
An optimal solution to \eqref{eq_Simple}
%, or equivalently \eqref{eq_c}-\eqref{eq_dual}, 
satisfies


%is determined by solving
%\begin{align}\label{eq_equation}
%\mathbb{E}[Y_i+Z_i] \!=\! \max\left(\frac{1}{f_{\max}}, \frac{\mathbb{E}[(W_{S_{i}+Y_i+Z_i}-W_{S_i})^4]}{2\beta}\right).\!
%\end{align}
%The optimal  value of \eqref{eq_Simple} is then given by \emph{
%\begin{align}\label{thm_3_obj}
%\mathsf{mmse}_{\text{opt}}=\frac{\mathbb{E}[(W_{S_{i}+Y_i+Z_i}-W_{S_i})^4]}{6\mathbb{E}[Y_i+Z_i] } + \mathbb{E}[Y].
%\end{align}}
\end{theorem}



Note that 
the expectations in \eqref{eq_equation} and \eqref{thm_3_obj} remain constant for all $i=1,2,\ldots$, as shown in \cite{Sun_reportISIT17}. Finally,  \eqref{eq_opt_stopping} is solved by using the optimal stopping rule developed in  \cite{Shiryaev1978}.
%\begin{proof}
%See Appendix \ref{app_solution_form}. 
%\end{proof}
%By this, 
% and the optimal $\alpha$ is given by \eqref{eq_equation}.

%\subsection{Per-sample Optimal Stopping Rule}


%Let us first pose \eqref{eq_opt_stopping} in the language of  optimal stopping.
%A continuous-time two-dimensional Markov chain $X_t$ on a probability space $(\mathbb{R}^2,\mathcal{F},\mathbb{P})$ is defined as follows:  Given the initial state $ X_0=x = (s,b)$, the state $X_t$ at time $t$ is  
%\begin{align}\label{eq_Markov}
%X_t= (s + t, b + W_t), 
%\end{align}
%where $\{W_t,t\geq 0\}$ is a standard Wiener process. 
%%Define $\mathbb{P}^x(A) = \mathbb{P}(A | X_0 = x)$ and $\mathbb{E}^x Z = \mathbb{E}(Z | X_0 = x)$, respectively, 
%%as the conditional probability of event $A$ and the conditional expectation of random variable $Z$ 
%%for given  initial state $X_0 =x$. 
%Define the $\sigma$-field $\mathcal{F}^{X}_t  = \sigma(X_{v}: v\in[0, t])$ and the {filtration} $\{\mathcal{F}^{X}_t ,t\geq0\}$ of the Markov chain $X_t$.
%A random variable $\tau: \mathbb{R}^2\rightarrow [0,\infty)$ is said to be a \emph{stopping time} of $X_t$ if $\{\tau \leq t\}\in \mathcal{F}^{X}_t $ {for all}~$t\geq0$. Let ${\mathfrak{M}}$ be the set of  square-integrable stopping times of $X_t$, i.e.,
%\begin{align}
%\mathfrak{M} = \{\tau \geq 0:  \{\tau\leq t\} \in \mathcal{F}^{X}_t , \mathbb{E}\left[\tau^2\right]<\infty\}.\nonumber
%\end{align}

%Let $\{\mathcal{F}(t),t\geq0\}$ be a \emph{filtration} of the process $\{X(t),t\geq 0\}$, that is, a family of $\sigma$-fields 
%$\mathcal{F}(t) = \sigma(X(s):0\leq s \leq t)$ such that $\mathcal{F}(s) \subset \mathcal{F}(t)  \subset \mathcal{F}$ for all $0\leq s< t$. 
%A random variable $\tau: \mathbb{R}^2\rightarrow [0,\infty]$ is said to be a \emph{stopping time} with respect to the filtration $\{\mathcal{F}(t),t\geq0\}$ if $\{\tau \leq t\}\in \mathcal{F}(t)$ {for all}~$t\geq0$.
%Let $\overline{\mathfrak{M}}$ be the set of all stopping times and $\mathfrak{M}$ be the set of all finite stopping times, i.e.,\begin{align}
%\mathfrak{M} = \{\tau\in \overline{\mathfrak{M}}: \mathbb{P}^x(\tau<\infty) = 1,~\forall~x\in \mathbb{R}^2\}.
%\end{align}
%Our goal is to solve the following optimal stopping problem:
%\begin{align}\label{eq_stop_prob}
%\sup_{\tau\in \mathfrak{M}}  \mathbb{E}^x g(X_\tau),
%\end{align}
%where the function $g: \mathbb{R}^2\rightarrow \mathbb{R}$ is defined as 
%\begin{align}\label{eq_fun}
%g(s,b) = - \frac{1}{2}b^4+\beta s 
%\end{align}
%with parameter $\beta \geq 0$, and $x$ is the initial state of the Markov chain $X(t)$. Note that \eqref{eq_stop_prob} reduces to \eqref{eq_opt_stopping}
%if the initial state is $ x=(Y_i,W_{S_{i}+Y_i}-W_{S_i})$,  and  $W_t$ is replaced by $W_{S_{i}+Y_i+t}-W_{S_i}$. 
%By using the optimal stopping theory of Markov chain \cite{Shiryaev1978,Peskir2006}, we establish the following result:
%\begin{theorem}\label{thm_optimal_stopping}
%For any initial state $(s,b)\in \mathbb{R}^2$, an optimal stopping time for solving \eqref{eq_stop_prob} is
%\begin{align}\label{eq_opt_stop_solution}
%\tau^* = \inf \left\{ t \geq 0:\! \left|b+W_t\right| \!\geq\! \sqrt{\beta}\right\}.
%\end{align}
%\end{theorem} 
%\begin{proof}
%See our technical report \cite{Sun_reportISIT17}.
%\end{proof}
%We will prove Theorem \ref{thm_optimal_stopping} by using the optimal stopping theory of Markov chain \cite{Shiryaev1978,Peskir2006}. To that end, 

%In order to prove Theorem \ref{thm_optimal_stopping}, let us define the function
%$u(x) = \mathbb{E}^x g(X_{\tau^*})$ and establish some properties of $u(x)$.
%
%\begin{lemma} \label{lem1_stop}
% $u(x)\geq g(x)$ for all $x\in \mathbb{R}^2$, and 
%\begin{align}
%u(s,b) = \left\{\begin{array}{l l} 
%\beta s- \frac{1}{2}b^4 , &\text{if}~ b^2 \geq \beta;
%\vspace{0.5em}\\
%\beta s+ \frac{1}{2} \beta ^2- \beta b^2 , &\text{if}~ b^2 < \beta.
%\end{array}\right.
%\end{align}
%\end{lemma} 
%\begin{proof}
%See Appendix \ref{app_optimal_stopping}. 
%\end{proof}
%
%A function $f(x)$ is said to be \emph{excessive} for the process $X_t$ if \cite{Shiryaev1978}
%\begin{align}
%\mathbb{E}^x f(X_t)\leq f(x),~\text{for all}~ t\geq 0, ~x\in \mathbb{R}^2.
%\end{align} 
%By using It\^{o} and Tanaka's formula in stochastic calculus, we can obtain
%\begin{lemma}\label{lem2_stop}
%The function $u(x)$ is excessive for the process $X_t$.
%\end{lemma} 

%
%\begin{proof}
%See Appendix \ref{app_optimal_stopping1}. 
%\end{proof}
%
%Now, we are ready to prove Theorem \ref{thm_optimal_stopping}. 
%\begin{proof}[Proof of Theorem \ref{thm_optimal_stopping}]
%In Lemma \ref{lem1_stop} and Lemma \ref{lem2_stop}, we have shown that $u(x)=\mathbb{E}^x g(X_{\tau^*})$ is an excessive function and $u(x)\geq g(x)$. In addition, it is known that $\mathbb{P}^x(\tau^*<\infty) = 1$ for all $x\in \mathbb{R}^2$ \cite[Theorem 8.5.3]{Durrettbook10}. These conditions, together with the Corollary to Theorem 1 in \cite[Section 3.3.1]{Shiryaev1978}, imply that $\tau^*$ is an optimal stopping time of \eqref{eq_stop_prob}. This completes the proof.
%\end{proof}


%An immediate consequence of Theorem \ref{thm_optimal_stopping} is
\begin{theorem}\label{coro_stop}
An optimal solution to \eqref{eq_opt_stopping} is
\begin{align}\label{eq_opt_stop_solution1}
Z_i = \inf \left\{ t \geq 0:\! \left|W_{S_i+Y_i+t}-W_{S_i}\right| \!\geq\! \sqrt{\beta}\right\},
\end{align}
and the expectations in \eqref{eq_equation} and \eqref{thm_3_obj} are then given by
\begin{align}
&\mathbb{E}[Y_i+Z_i] = \mathbb{E}[\max(\beta,W_Y^2)],\label{eq_expression0}\\
&\mathbb{E}[(W_{S_{i}+Y_i+Z_i}-W_{S_i})^4] = \mathbb{E}[\max(\beta^2,W_Y^4)].\label{eq_expression}
\end{align}
\end{theorem}
Combining Theorem \ref{thm_solution_form} and Theorem \ref{coro_stop}, Theorem~\ref{thm_1} follows.}
%Finally, \eqref{eq_expression0} and \eqref{eq_expression} are proven in Appendix \ref{app_expression}. 
%This completes the proof of Theorem \ref{thm_1}.


